Semantic Frame Parsing for Information Extraction : the CALOR corpus

This paper presents a publicly available corpus of French encyclopedic history texts annotated according to the Berkeley FrameNet formalism. The main difference in our approach compared to previous works on semantic parsing with FrameNet is that we are not interested here in full text parsing but rather on partial parsing. The goal is to select from the FrameNet resources the minimal set of frames that are going to be useful for the applicative framework targeted, in our case Information Extraction from encyclopedic documents. Such an approach leverages the manual annotation of larger corpora than those obtained through full text parsing and therefore opens the door to alternative methods for Frame parsing than those used so far on the FrameNet 1.5 benchmark corpus. The approaches compared in this study rely on an integrated sequence labeling model which jointly optimizes frame identification and semantic role segmentation and identification. The models compared are CRFs and multitasks bi-LSTMs.

==> partial_parsing.tex <==
\section{Full-text parsing \textit{vs.} partial parsing}

\begin{figure*}[htbp] 
  \includegraphics[width=1\linewidth]{Figures/exemple_frame.pdf}
  \caption{Example of Frame multilabel annotation}
  \label{fig:exemple_frame}
\end{figure*}

Two kinds of parsing can be done with a Semantic Frame model: \textit{full text parsing} where each word in a sentence is analyzed to check if it can be a LU evoking a frame; and \textit{partial parsing} where only a subset of frames and LUs is considered, according to their relevance for a given applicative framework.
Annotating all the possible LUs and frames in a sentence is a very difficult (and expensive) task for human annotators, therefore there are very little corpora annotated this way. Moreover not many languages have such resources.
Most of previous work in semantic frame parsing that has been done with a \textit{full text parsing} approach have used the benchmark corpus FrameNet 1.5. Although the size of this benchmark is relatively big, a lot of frames have a very small number of occurrences in the corpus. This is due to the very large number of frames considered in the semantic model and this makes this corpus particularly challenging for machine learning methods.

On the contrary \textit{partial parsing} can be made on large corpora at a reasonably low cost: because the amount of frames and LUs is limited, the annotators can focus only on a few words for each sentence, making the task much easier than full parsing. Corpus obtained this way contain much more examples for each frame, opening the door to more machine learning methods than full parsing.

From an applicative point of view, \textit{partial parsing} is also a more realistic option. Although the different senses from the FrameNet model are generic, models trained on the FrameNet 1.5. corpus are not. Assuming that a full text annotation will be available for each new applicative domain is not an option. Moreover a lot of applicative frameworks using semantic models such as frames, like the Information Extraction framework considered in this study, are not interested in full parses but on the contrary only in some specific senses related to the domain targeted.

An example of this kind of annotation scheme is given in figure \ref{fig:exemple_frame}. As we can see, only two words as considered as lexical units in the sentence: \texttt{decide}, which triggers the frame \texttt{Deciding} and \texttt{order} triggering the frame \texttt{Request}.



==> related_work.tex <==
\section{Related work}
\label{sec:previouswork}


As mentioned in the previous section, most previous work on Semantic Frame parsing have been done following a \textit{full text parsing approach} on FrameNet 1.5 data.
An overview of statistical methods used in this context can be found in~\cite{das2014statistical}.
State-of-art systems, such as~\cite{hermann2014semantic}, implement a multi-step approach: firstly a classification process is in charge of deciding if a potential frame trigger is a Lexical Unit triggering a given frame; secondly, once a frame is hypothetized, candidates for frame elements are produced, often thanks to heuristics on the syntactic analysis of the sentence, then labeled as a classification task with semantic role categories; finally a global model is applied in order to filter and link FEs together in order to guarantee some coherence in the annotation produced.
Systems differ from the way these global constraints are integrated into the parsing process: hard structural constraints with an integer linear program (ILP) approach for~\cite{hermann2014semantic}; imitation learning for~\cite{wolfe2016study} or dynamic programming for semantic role labeling in~\cite{tackstrom2015efficient}.
All these methods take as input a structured representation of the sentences to process, obtained through a syntactic analysis phase, often realized thanks to a syntactic dependency parser.
In addition to provide features for the different classifiers involved, these syntactic parses are necessary in order to select frame element candidates in a sentence once a frame is detected.

In addition to the fact that we are doing partial parsing rather than full text parsing, the approaches proposed in this study differ significantly from these previous studies on two key characteristics: firstly we use sequence labeling methods for performing \textit{jointly} frame and frame element detection; secondly we don't assume than a structured input is needed to run our systems.
Indeed we present experiments where we compare performance with and without syntactic features, showing than for one of our system the loss in performance is rather small when only words are given as input.


% \begin{itemize}
% \item \cite{wolfe2016study} \textit{A Study of Imitation Learning Methods for Semantic Role Labeling} : global features on top of local processes
% \item \cite{hermann2014semantic} \textit{Semantic Frame Identification with Distributed Word Representations} : state of the art with embeddings and NN
% \item \cite{tackstrom2015efficient} \textit{Efficient Inference and Structured Learning for Semantic Role Labeling} : using dynamic programming for semantic frame parsing
% \item \cite{kshirsagar2015frame} \textit{Frame-Semantic Role Labeling with Heterogeneous Annotations} : limitation of FrameNet resources, how to augment them?
% %\item \textit{Deep Multitask Learning for Semantic Dependency Parsing} : the latest news on semantic frame parsing !! deep, no syntax, good results .... not yet published (arxiv)
% \item \cite{hartmannout} \textit{Out-of-domain FrameNet Semantic Role Labeling} : domain adaptation
% \end{itemize}

